Surface Analysis with Vision Transformers

The extension of convolutional neural networks (CNNs) to non-Euclidean geometries has led to multiple frameworks for studying manifolds. Many of those methods have shown design limitations resulting in poor modelling of long-range associations, as the generalisation of convolutions to irregular surfaces is non-trivial. Recent state-of-the-art performance of Vision Transformers (ViTs) demonstrates that a general-purpose architecture, which implements self-attention, could replace the local feature learning operations of CNNs. Motivated by the success of attention-modelling in computer vision, we extend ViTs to surfaces by reformulating the task of surface learning as a sequence-to-sequence problem and propose a patching mechanism for surface meshes. We validate the performance of the proposed Surface Vision Transformer (SiT) on two brain age prediction tasks in the developing Human Connectome Project (dHCP) dataset and investigate the impact of pre-training on model performance. Experiments show that the SiT outperforms many surface CNNs, while indicating some evidence of general transformation invariance. Code available at https://github.com/metrics-lab/surface-vision-transformers

==> CVPR - t4v workshop - SiT - camera ready (1)/cardiac.tex <==

\subsection{SCOT-HEART: high-calcium classification}
\paragraph{Data}

\begin{figure}[!t]
  \centering
\makebox[\linewidth]{%to center the image
	\includegraphics[width=0.9\columnwidth]{figures/cardiac2.001.jpeg}}
\caption{Biventricular coarse mesh (a), and final mesh (b), longitudinal view. The green, purple, and black surfaces are the LV endocardial, RV endocardial and biventricular epicardial surfaces.}
\label{figure:cardiac}
\end{figure}
Data for this experiment consisted of biventricular surface meshes, comprising endocardial and epicardial surfaces, customised to patients with suspected coronary artery disease, who participated in the Scottish Computed Tomography of the Heart (SCOT-HEART) trial \cite{DE.Newby2018}. Coronary artery calcium score (CACS) was used as a surrogate biomarker, since it is known to be highly predictive of adverse cardiovascular events and associated with changes in heart geometry \cite{M.Budoff2018,H.Bakhshi2017}. A total of 615 cardiac meshes were used (248 healthy participants with CASC $<300$ AU, and 367 high-CACS participants with CACS $>300$ AU). Figure \ref{figure:cardiac} (b) shows an element of the coarse mesh and for each element endocardial and epicardial surfaces there are $25\times 2=50$ corresponding vertices from the final mesh.

Coronary computed tomography angiography (CCTA) images part of the SCOT-HEART trial \cite{DE.Newby2018} were first segmented using a neural network algorithm \cite{H.Xu2021} and then biventricular meshes were fitted to the surface points extracted from the segmentation results by deforming a finite element model \cite{C.Mauger2019}. The biventricular subdivision surface model was initiated with a control mesh consisting of 388 vertices and 180 elements. A final mesh was obtained after subdividing the control mesh twice using the Catmull-Clark algorithm, giving $5\times 5=25$ vertices for each surface patch \cite{C.Mauger2018} as shown in Figure \ref{figure:cardiac}, redrawn from \cite{C.Mauger2018}. This resulted in a template mesh of 354 patches, where patches were subsequently merged in pairs to generate 177 larger patches (with 50 vertices per patch) which were then used for training. 

\paragraph{Results}

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lc}
        \toprule
         \textbf{Methods} &  \textbf{AUC} \\
        \midrule
        Logistic regression & 0.750 \\
        \midrule
        SiT-tiny &  0.738 $\pm$ 0.04 \\
        SiT-small& 0.742 $\pm$ 0.03\\
        \bottomrule
        
        \\
\end{tabular}
\caption{Cardiac mesh classification results. SiT-tin was trained following a five folds cross-validation, and compared against a baseline logistic regression.}
\centering
\label{Table:cardiac_results}
\end{table}

The performance of the SiT was benchmarked for the task of cardiac mesh classification between healthy and high CASC against a baseline logistic regression model, using standard LV and RV volumes and LV mass as predictors, with five-fold cross-validation. A mean cardiac shape was constructed using Procrustes alignment and the displacement of the biventricular meshes from the mean shape ($dx, dy, dz$) and the wall thickness ($t$) forms the 4 feature channels used for the \emph{SiT} models. Models were trained using five-fold cross validation and best performance was achieved using Adam optimiser and a learning rate of $3e^{-4}$. 
Best performances (reported in Table \ref{Table:cardiac_results}) were obtained using the larger patches of 50 vertices. SiT models with smaller patches overfit dramatically, and would probably benefit from specific data augmentation and adaption of the embedding dimension to account for the small number of vertices in the patch sequence. \emph{SiT} models obtained good performances using mesh displacement and wall thickness, similar to the ones obtained with logistic regression used as standard clinical metrics.


==> cardiac.tex <==

\subsection{SCOT-HEART: high-calcium classification}
\paragraph{Data}

\begin{figure}[!t]
  \centering
\makebox[\linewidth]{%to center the image
	\includegraphics[width=0.9\columnwidth]{figures/cardiac2.001.jpeg}}
\caption{Biventricular coarse mesh (a), and final mesh (b), longitudinal view. The green, purple, and black surfaces are the LV endocardial, RV endocardial and biventricular epicardial surfaces.}
\label{figure:cardiac}
\end{figure}
Data for this experiment consisted of biventricular surface meshes, comprising endocardial and epicardial surfaces, customised to patients with suspected coronary artery disease, who participated in the Scottish Computed Tomography of the Heart (SCOT-HEART) trial \cite{DE.Newby2018}. Coronary artery calcium score (CACS) was used as a surrogate biomarker, since it is known to be highly predictive of adverse cardiovascular events and associated with changes in heart geometry \cite{M.Budoff2018,H.Bakhshi2017}. A total of 615 cardiac meshes were used (248 healthy participants with CASC $<300$ AU, and 367 high-CACS participants with CACS $>300$ AU). Figure \ref{figure:cardiac} (b) shows an element of the coarse mesh and for each element endocardial and epicardial surfaces there are $25\times 2=50$ corresponding vertices from the final mesh.

Coronary computed tomography angiography (CCTA) images part of the SCOT-HEART trial \cite{DE.Newby2018} were first segmented using a neural network algorithm \cite{H.Xu2021} and then biventricular meshes were fitted to the surface points extracted from the segmentation results by deforming a finite element model \cite{C.Mauger2019}. The biventricular subdivision surface model was initiated with a control mesh consisting of 388 vertices and 180 elements. A final mesh was obtained after subdividing the control mesh twice using the Catmull-Clark algorithm, giving $5\times 5=25$ vertices for each surface patch \cite{C.Mauger2018} as shown in Figure \ref{figure:cardiac}, redrawn from \cite{C.Mauger2018}. This resulted in a template mesh of 354 patches, where patches were subsequently merged in pairs to generate 177 larger patches (with 50 vertices per patch) which were then used for training. 

\paragraph{Results}

\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lc}
        \toprule
         \textbf{Methods} &  \textbf{AUC} \\
        \midrule
        Logistic regression & 0.750 \\
        \midrule
        SiT-tiny &  0.738 $\pm$ 0.04 \\
        SiT-small& 0.742 $\pm$ 0.03\\
        \bottomrule
        
        \\
\end{tabular}
\caption{Cardiac mesh classification results. SiT-tin was trained following a five folds cross-validation, and compared against a baseline logistic regression.}
\centering
\label{Table:cardiac_results}
\end{table}

The performance of the SiT was benchmarked for the task of cardiac mesh classification between healthy and high CASC against a baseline logistic regression model, using standard LV and RV volumes and LV mass as predictors, with five-fold cross-validation. A mean cardiac shape was constructed using Procrustes alignment and the displacement of the biventricular meshes from the mean shape ($dx, dy, dz$) and the wall thickness ($t$) forms the 4 feature channels used for the \emph{SiT} models. Models were trained using five-fold cross validation and best performance was achieved using Adam optimiser and a learning rate of $3e^{-4}$. 
Best performances (reported in Table \ref{Table:cardiac_results}) were obtained using the larger patches of 50 vertices. SiT models with smaller patches overfit dramatically, and would probably benefit from specific data augmentation and adaption of the embedding dimension to account for the small number of vertices in the patch sequence. \emph{SiT} models obtained good performances using mesh displacement and wall thickness, similar to the ones obtained with logistic regression used as standard clinical metrics.

